Free Vibrations of Axisymmetric Shells: Parabolic and Elliptic cases

Approximate eigenpairs (quasimodes) of axisymmetric thin elastic domains with laterally clamped boundary conditions (Lam{\'e} system) are determined by an asymptotic analysis as the thickness ($2\varepsilon$) tends to zero. The departing point is the Koiter shell model that we reduce by asymptotic analysis to a scalar modelthat depends on two parameters: the angular frequency $k$ and the half-thickness $\varepsilon$. Optimizing $k$ for each chosen $\varepsilon$, we find power laws for $k$ in function of $\varepsilon$ that provide the smallest eigenvalues of the scalar reductions.Corresponding eigenpairs generate quasimodes for the 3D Lam{\'e} system by means of several reconstruction operators, including boundary layer terms. Numerical experiments demonstrate that in many cases the constructed eigenpair corresponds to the first eigenpair of the Lam{\'e} system.Geometrical conditions are necessary to this approach: The Gaussian curvature has to be nonnegative and the azimuthal curvature has to dominate the meridian curvature in any point of the midsurface. In this case, the first eigenvector admits progressively larger oscillation in the angular variable as $\varepsilon$ tends to $0$. Its angular frequency exhibits a power law relationof the form $k=\gamma \varepsilon^{-\beta}$ with $\beta=\frac14$ in the parabolic case (cylinders and trimmed cones), and the various $\beta$s $\frac25$, $\frac37$, and $\frac13$ in the elliptic case.For these cases where the mathematical analysis is applicable, numerical examples that illustrate the theoretical results are presented.

==> kmodBDHL.tex <==
$\varepsilon$  &  B  &  B  &  D  &  D  &  H  &  H  &  L  &  L \\  
0.20000  &   2  &   3.2  &   1  &   1.5  &   1  &   1.4  &   1  &   1.7\\ 
0.10000  &   2  &   3.8  &   2  &   1.8  &   2  &   1.9  &   2  &   2.3\\ 
0.05000  &   3  &   4.5  &   2  &   2.3  &   2  &   2.5  &   2  &   3.1\\ 
0.02000  &   4  &   5.6  &   3  &   3.2  &   4  &   3.6  &   3  &   4.6\\ 
0.01000  &   6  &   6.7  &   4  &   4.0  &   5  &   4.8  &   4  &   6.1\\ 
0.00500  &   7  &   8.0  &   5  &   5.0  &   6  &   6.3  &   5  &   8.2\\ 
0.00200  &   9  &  10.0  &   7  &   6.8  &   9  &   9.1  &  10  &  12.2\\ 
0.00100  &  11  &  11.9  &   9  &   8.6  &  12  &  12.0  &  15  &  16.4\\ 
0.00050  &  14  &  14.2  &  11  &  10.8  &  16  &  15.9  &  21  &  22.1\\ 
0.00020  &  17  &  17.9  &  15  &  14.7  &  23  &  22.9  &  32  &  32.7\\ 
0.00010  &  21  &  21.2  &  18  &  18.5  &  30  &  30.2  &  43  &  44.1\\ 
0.00005  &  --  &  --    &  24  &  23.3  &  40  &  39.9  &  59  &  59.3\\ 

